CURI: A Benchmark for Productive Concept Learning Under Uncertainty

Humans can learn and reason under substantial uncertainty in a space of infinitely many concepts, including structured relational concepts ("a scene with objects that have the same color") and ad-hoc categories defined through goals ("objects that could fall on one's head"). In contrast, standard classification benchmarks: 1) consider only a fixed set of category labels, 2) do not evaluate compositional concept learning and 3) do not explicitly capture a notion of reasoning under uncertainty. We introduce a new few-shot, meta-learning benchmark, Compositional Reasoning Under Uncertainty (CURI) to bridge this gap. CURI evaluates different aspects of productive and systematic generalization, including abstract understandings of disentangling, productive generalization, learning boolean operations, variable binding, etc. Importantly, it also defines a model-independent "compositionality gap" to evaluate the difficulty of generalizing out-of-distribution along each of these axes. Extensive evaluations across a range of modeling choices spanning different modalities (image, schemas, and sounds), splits, privileged auxiliary concept information, and choices of negatives reveal substantial scope for modeling advances on the proposed task. All code and datasets will be available online.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/archive_intro.tex <==
\iffalse
Abstraction
\begin{enumerate}
\item One of the central challenges in artificial intelligence is to perform appropriate abstraction
\item As humans, we are able to think in a really flexible manner about the objects and the properties we see
in our environment
\item For example, given a set of objects ``apple, rain, and leaves'', we are able to abstract that the underlying
concept has something to do with ``things that could fall on one's head''
\item On the other hand, if we saw a set of objects ``apple, orange, bananas'', one might perform a different
abstraction, believing that one was referring to the set of ``fruits that one can eat for breakfast''.
\end{enumerate}

Abstraction and Representation Learning
\begin{enumerate}
    \item Beyond learning concepts in a felxible manner, the notion of abstraction is also important
    for representation learning
    \item For example, a model that learns the right abstractions say, when playing ping pong would
    realize that the color of the paddle does not matter, but it might matter when picking a paddle
    that person likes, for example
    \item Thus, models that demonstrate intelligent behavior need to demonstrate an ability to capture
    the different facets of a perceptual input that one might be interested in
\end{enumerate}

Abstraction and Language of Thought
\begin{enumerate}
    \item In order to make progress on the problem of learning flexible abstractions, we study a concept
    lerning task in the space of realizations from a language of thought~\citep{Piantadosi2016-bx}
    \item We study the capacity of models to perform such abstraction, and to learn (and generalize)
in an essentially infi flexible relational and quantificational
concepts~\citep{Lake2017-pp,Piantadosi2016-bx,Kemp2009-sn}
    \item Formally, a language of thought is {... ADD..}
    \item The compositionality and structure in the lagnuage of thought
    allows us to flexibly sample concepts (and their realizations) from an exponential space of 
    possible concepts
    \item Such a learning setting has been extensively studied in previous works in cognitive science with humans
    ~\citep{Piantadosi2016-bx,Kemp2009-sn}
    \item In this paper, we test if few-shot learning approaches can learn to perform abstraction
\end{enumerate}

Task Description
\begin{enumerate}
    \item Concretely, we propose a task where given a set of images belonging to an underlying 
\end{enumerate}

Findings
\fi
People can reason in more abstract and flexible ways than today's AI systems, suggesting that ``abstraction'' is a factor in the
gap between human and machine understanding \citep{Lake2017-pp,Ho2019-gt}. 
People not only understand the world in terms of common categories ---such as ``fruit'' or ``furniture''--- they can also induce
spontaneous or ``ad hoc'' categories based on their context and goals \citep{Barsalou1983-ud}. For instance, people can reason
about ``things to take from one's home in a fire'' (children, pets, keepsakes, etc.) or ``objects that could fall on one's head''
(apples, rain, leaves, etc.), showing that people's conceptual repertoires are not limited to a small number of fixed sets.
The productivity of human concepts is similarly evident in human language and thought \citep{Chomsky1957,Fodor1975}.
People can reason about noun compounds such as ``apple car'' or ``apartment dog,'' even without ever entertaining these complex
concepts before \citep{Murphy1988,Murphy2002}.

Children must learn how to combine simple concepts (``apple'' and ``red'') with relations
(``big'' and ``above'') to understand
complex meanings, such as ``the smallest apple is red'' or
``the red apples are above the green ones''~\citep{Montague1970}.
\rama{Moreover, we condense experiences into such concepts and theories derived from them to understand
and analyze our everyday experiences.
Such an ability is not only
fundamental to human learning, but is also potentially useful for a number of challenges
in machine learning such as generalization to out of distribution data, planning,
reasoning, grounded language learning, and creativity~\citep{Mordatch2018-gn}.}

%problems such as 
%Such capabilities highlight the productivity of human conceptual learning and reasoning compared
%to standard machine learning systems
%that learn to recognize only a fixed,
%finite set of labeled classes~\citep{imagenet}, \rama{and find it difficult to
%perform systematic, out of distribution generalization~\citep{Lake2017-ij,Agrawal2017-qw,imagination,Arjovsky2019-qc}
%that we need for productive abstractions.}
%\ari{[*] This last point, which contrasts the cog
%sci perspective
%of flexible reasoning with ML models is critical for the reader to understand and buy into. If they're not convinced that this
%is important and that our current model is lacking, the paper isn't really worthwhile. I think the above convincingly makes the
%point that flexible reasoning is critical in humans, but we should spend more time here unpacking how current models are lacking.}
% For example, given a concept learning task where one is given the words
% ``apple, rain, leaves'' one might reason that the underlying concept here is something to do with ``things that
% could fall on one's head.'' On the other hand, if we saw a set of objects ``apples, oranges, bananas'', one would
% infer a different concept of ``fruits''. Thus, depending upon the context, we are able to adaptively assign
% or reason about different, productive
% abstractions or concepts associated with an entity (say ``apples'').
% Such a capability
% in humans has been extensively studied in the cognitive science literature on ad hoc categorization~\citep{Barsalou1983-ud},
% \rama{where such categories typically emerge from abstract goals and functions.}

% This paper examines the productive abstraction capabilities of modern machine learning algorithms.
% This is interesting not only from the perspective of building machines with human-like capabilities but serves as a test of
% deep representation learning (and broadly machine learning),
% in terms of being able to form different abstractions (or ways of thinking and reasoning) about an observed entity.
\begin{figure}\label{fig:teaser}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser.pdf}
    \caption{\noindent\textbf{Productive Abstraction Inference:} Given a few examples of positive and negative
    images for an unseen, novel concept such as ``There exists a blue object and the rest of the objects are cylinders'', the goal for
    a model is to output an accurate classifier, demonstrating an ability to `abstract out' the underlying concept
    from samples.}
\end{figure}
\rama{In this work, we explicitly study the ability of machine learning systems to collate (or abstract)
experiences into concepts and theories about the world.}
Concretely, we contribute a large-scale
benchmark for few-shot learning of relational concepts in an
essentially unbounded, compositional conceptual space.
\rama{We situate ourselves in the general framework of meta learning~\citep{Lake2019-tu,Finn2017-bw}
where we hope to teach models inductive biases about relevant concepts and theories in the world,
such that the model is able to perform productive abstraction for a novel experience never
seen before during training time (\cref{fig:teaser}).
}
Traditional classification problems use a fixed set of classes and require applying
familiar classes to novel images during
generalization ~\citep{imagenet}. One-shot classification and meta-learning require generalizing outside the set of classes seen
during training \cite{FeiFeiFergus2006,Vinyals2016-ri,LakeOmniglotProgress}, but current benchmarks focus on relatively simple
concepts compared to the more structured, relational concepts that characterize distinctively human abstractions.  We utilize the
compositionality of language-like representations to create an essentially unbounded, richly compositional space of concepts.
\rama{Specifically, we are inspired by the ``language of thought'' hypothesis which posits that humans have a structured,
compositional representation system that provides a substrate for thinking~\citep{Piantadosi2016-bx,Fodor1975,Boole1854-hc}
and has been used for cognitive modeling to study how people make ``conceptual leaps'' when learning structued concepts
~\citep{Goodman2008a,Kemp2012,Goodman2014,Piantadosi2016-bx}, counting and learning
quantifiers and language~\citep{Piantadosi_thesis}.}
 \ari{[*] Need a clear definition of language of thought here.
This isn't a common term for the ML audience. We might actually want to move this sentence into the first paragraph.}. Our benchmark
also utilizes a language of thought for specifying the conceptual space, using a variant most related to \citet{Piantadosi2016} equipped
with a rich set of relational and quantification operators.
In addition, we stress test our baseline models by exploring different systematic settings for generalization to check
the ability of machine learning models to extrapolate (or ``reason'') beyond the data that they have seen.
While previous work~\citep{Barrett2018-qr,Agrawal2017-qw,LakeBaroni2018} has studied and proposed such systematic splits
\rama{(with different concepts being provided in training and testing)} in other
contexts, \rama{we provide the first such split in the context of image classification and concept learning.
Importantly, we are also able to quantify and benchmark the difficulty of 
a split, providing an indication of
a `compositionality gap' which must be overcome for generalization which makes it easier to evaluate and reliably measure
progress.}
\ari{[*] This point doesn't really come through clearly}.

%\ari{Would be good to emphasize here a bit more what's missing in the current literature}
Concretely, we situate the task in the realm of meta-learning~\citep{Schmidhuber1996-am,LakeOmniglotProgress,meta_dataset}.
At inference time, a model is given a small
collection
of observations and labels $D_{supp} = \{x^i, y^i\}_{i=1}^{N}$ ~\cref{fig:teaser}, where the label indicates whether an observation
$x_i$ is true for the concept of interest $c^*$. Given this, the task for a model is to infer a classification
rule for novel datapoints at test time. The key difference from prior work~\citep{LakeOmniglotProgress,meta_dataset}
is that the concepts $c^*$ are drawn from a rich, structured
language of thought concept space. For example, one is asked to infer a concept (and a classifier) such as
\texttt{``count of objects with same material is greater than count of objects with same shape''}, given
a background knowledge that counts, shapes, and materials exist in the world (from having seen other concepts sampled
from the language of thought), but having never seen anything other than the small set of examples
in $D_{supp}$ for $c^*$. While traditional meta-learning approaches relate to
learning a new task faster by speeding-up optimization~\citep{Ravi2016-vg,Finn2017-bw} or feature-reuse and
adaptation~\citep{Snell2017-rl}, in our task there is an underlying language of thought, which if understood
can help constrain the space of possible abstractions, and achieve faster adaptation. Since we are situated
at the intersection of language of thought and meta-learning, we call the dataset~\pcl.

We further probe and explore different generalization regimes for abstraction by creating structured
splits that utilize the language of thought representation to create test sets of varying degree of
difficulty by carefully choosing which concepts $c^*$ are withheld from the training stage
of the models. \todo{Our analysis reveals..}. One can view set of experiments is in line with more recent work
in machine learning around systematicity~\citep{Fodor1988-wb,LakeBaroni2018}, applied to the problem of few-shot
learning, which is a novel and interesting test-ground for systematic generalization. Further, we provide
the dataset in three modalities (image, symbolic specifications, and sounds) to compare and contrast
the difficulty of performing abstraction based on the input representation. 

\noindent\textbf{Contributions:}
1) We propose a new task and dataset, called \pcl, to systematically test the ability of models to form
ad-hoc abstractions; 2) We characterize the degree of difficulty in performing abstraction when the test
and training tasks differ systematically; 3) We provide the dataset in three different modalities,
where we render $x$ as either an image, a symbolic
scene specification or as a sound, and analyze the representations across modalities; 4) We present evaluation
metrics and baseline models to facilitate future work on abstraction in compositional, relational concept learning. \todo{Analysis contribution}

==> sections/archive_related.tex <==
% Our work draws on related threads of research across cognitive science and machine learning.

\noindent\textbf{Concept Learning}. 
\brenden{I suggest we cut this entire ``concept learning'' section. It's redundant with the introduction and we need to save space. We'll need to find a place for Mordatch, but all the other papers are cited already} \ari{I agree, but perhaps move to expanded related work section in appendix?} 
Given their foundational importance to intelligent behavior~\citep{Murphy_big_book_concepts}, concept
learning has received a lot of attention from both human as well as machine learning perspectives.
In the cognitive science literature, most closely connected work to ours are~\citep{Goodman2008a,Kemp2012,Goodman2014
,Piantadosi2016-bx} which
work on modeling human concept acquisition using probabilistic context free grammars over a `language
of thought' that provides a convenient modeling tool to combine basic concepts or primitives
(such as shapes, colors, \etc)
into more abstract, high level concepts (``there exists an object whose color is blue and shape circle'').
The compound concept space used in this work is highly inspired by the language of thought used by~\citet{Piantadosi2016-bx}.

In the machine learning domain, recent work from~\citet{imagination,Higgins2017-wa,Du2020-oj} studies how to
build joint conceptual representations of images and words, which allow one to generate or `imagine'
novel concepts specified in text. In contrast
to these works which are primarily interested in generative modeling, in this work we are interested
in the abduction of plausible concepts underlying observed episodes.
Other work builds energy based models~\citep{Mordatch2018-gn}
for concept learning, where
more complex concepts generated by arithmetic operations on energies of simpler concepts, which is used
to generate and identify concepts in simple settings. We share the same motivations as this work,
with a greater emphasis on creating a benchmark for abstraction/identification of more complex concepts
than can be currently handled by the energy based framework from~\citep{Mordatch2018-gn}\todo{verify}.
\todo{ILP and version spaces}

\noindent\textbf{Analogical Reasoning}. \brenden{This can be made much more concise to save room} Finally, recent work in machine
learning studies analogical reasoning, where one has to identify
abstract patterns~\citep{Santoro2016-ug,Barrett2018-xv,Hill2019-as} in Raven's matrices style IQ tests and apply them 
to novel perceptual inputs to guess the correct completion of a sequence. We are interested in a related,
but different problem of inducing abstract concepts from experiential data, as opposed to solving IQ tests.
In some sense, we view abstraction as a sub-task of abstract analogical reasoning, and focus on making
progress on the abstraction piece instead of combining it with analogies.
Finally, we build on the systematic splits introduced in context of Raven's matrices to reason
about compositionality gaps indicating the difficulty of abstraction. \todo{Not sure if we should mention
details like meta learning, multimodality, etc which to me are less important.}

% \iffalse
% Our work is closely related,
% in the sense that both approaches are interested in measuring abstraction, but our concept space is more
% structured and complicated, mimicking closely the language of thought posited by~\citep{Piantadosi2016-bx}.
% \rama{While~\citet{Santoro2016-ug} are interested in abstract analogical reasoning, we study the more
% atomic problem of productive abstraction, and provide a benchmark with multiple modalities, splits and compositionality
% gaps to make systematic progress on it. Finally, we situate ourselves in the meta-learning context, looking
% to study if the language of thought can be acquired as an inductive bias to aid low-shot classification
% while~\citet{Santoro2016-ug} situate themselves in the traditional classification setup.}
% \ari{[*] expand on differences a bit more here: meta-learning vs. typical classification, multi-modality, etc.}
% \fi

% \iffalse
% \noindent\textbf{Few-shot Learning}. Following the success of convolutional neural networks
% on the ImageNet classification task~\citep{imagenet}, there has been substantial interest in
% developing techniques for few-shot recognition~\citep{LakeOmniglotProgress,Vinyals2016-ri,Hariharan2017-mp,
% Wang2018-qe}, where the goal is to learn a generalizable classifier from a very limited set of examples. Most of the approaches to few-shot learning 
% are evaluated on handwritten characters~\citep{Lake2019-tu} or ImageNet images~\citep{imagenet,Vinyals2016-ri,
% Hariharan2017-mp} with standard classification label spaces, while here  we are interested in compositionally and relationally rich label spaces.
% \fi

\noindent\textbf{Meta-Learning}. \brenden{I also think this whole section on ``meta learning'' can be cut as we discuss the key points in the introduction already. we should move some of these meta-learning references to the intro, so no one is left out.} A popular class of approaches for few-shot learning involve meta-learning
or learning to learn. The key idea in such approaches is to build a strong inductive bias for the model
family (or the optimization) used for fitting a model in the few-shot phase from a family of related tasks.
Popular meta-learning approaches support learning through nearest neighbours~\citep{Vinyals2016-ri}, protoypes~\citep{Snell2017-rl,meta_dataset}, good initializations
for optimization~\citep{Finn2017-bw}, or memory-augmented neural networks~\citep{Santoro2016-ug,LakeMeta2019}, among others. In this 
paper, we use the prototypical network framework to evaluate different choices of models that one could
use for the meta-learning task \citep{Snell2017-rl}. While previous papers evaluated their
models on datasets designed for image classification such as mini-ImageNet~\citep{Vinyals2016-ri} or Omniglot~\citep{Lake2017-ij}, in this work we introduce a new
dataset specifically designed to study productive abstraction in the framework of meta-learning.
The \pcl dataset focuses on a rich, compositional, relational space of concepts as opposed to the rigidly hierarchical
concept space of standard image classification datasets.

Recently,~\citet{meta_dataset} proposed a novel benchmark for evaluating
meta learning models, with the key differences that the proposed benchmark uses taxonomic structure
in ImageNet and Omniglot, and evaluates models on different datasets than they used for meta-traning (e.g., training on ImageNet and evaluating on Omniglot), analyzing the degree to which the procedure for ``learning to learn'' generalizes.
Our work is also a proposal for evaluating meta-learning approaches, but our goal is explicitly to understand
the extent to which models are able to generalize to compositionally novel concepts in a high level semantic compound concept space,
as opposed to testing to what extent the ``learning to learn'' generalizes across different datasets.

\noindent\textbf{Other learning settings}:\brenden{Is the literature on zero-shot learning relevant at all to our paper? It would be nice to cite Andreas and CLEVR elsewhere earlier, but otherwise I think this can all be cut too.} Our work is related to some other learning settings previously
explored in the literature. Open set recognition~\citep{Scheirer2013-ho} focuses on the problem of identifying
unknown unknown categories (which have never been seen at training time) from the known known categories presented
to a model at training time. Different from open set recognition, our goal here is at test time to learn a new
classifier for an unknown unknown category, as opposed to marking an unknown unknown category as such \brenden{Why call this "unknown unknown" rather than just "novel"?}. Zero-shot
learning~\citep{Lampert2014-qo} utilizes side information to learn new categories from scratch, by essentially learning a mapping from
semantic information to the weights of a classifier. Different from zero shot learning, the (optional) input of 
the hypothesis (or program) corresponding to the concept we want to learn is not available at test-time, making
it necessary to perform abstraction of the concept from the examples in a support set, as opposed to any side
information. Most related to our proposal,
\citet{Andreas2017-yp} propose a learning setup where one treats language as a latent variable, inducing
novel classifiers from examples via the space of natural language. Thus in some sense, the natural language acts as a
bottleneck, restricting the space of functions and hypotheses. While the goal of~\citet{Andreas2017-yp}
is to show that language can be thought
of as a latent variable and used for classification, our goal is not to demonstrate that language can be used in such
a manner, but instead to propose a benchmark with systematic splits to test the extent to which
models perform abstractions. Finally, the CLEVR benchmark~\citep{Johnson2016_clevr} proposes compositional splits
for visual question answering, where a differrent distribution of questions are asked at test time about images.
We use the rendering engine from this work in order to render the scenes in the~\pcl dataset. However, our focus
is not on question answering, but on compound concept abstraction from observations.

==> sections/broader_impact.tex <==
\section*{Broader Impact}
People are natural compositional learners and reasoners, yet the best machine classifiers struggle with compositionality. We introduce a new benchmark and  ``compositionality gap'' measure for catalyzing research in this area. Advances in machine compositional learning could lead to more robust AI systems and more fluid human-machine interaction. We do not anticipate that our work will advantage or disadvantage any particular group.

% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare 
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}



==> sections/discussion.tex <==



==> sections/intro_new.tex <==
% People can reason in more productive and flexible ways than today's AI systems, understanding completely novel concepts and expressions \citep{Lake2017-pp,Ho2019-gt}.
% \ari{We still don't have a definition for productive anywhere here. I really think we have to define it in some way. Alternative suggestion: "People can reason flexibly, using a limited set of experiences to produce and reason about a large set of novel expressions and concepts, yet today's AI systems lack this ability."}
Human concept learning is more flexible than today's AI systems. Human conceptual knowledge is \emph{productive}: people can understand and generate novel concepts through compositions of existing concepts (``an apartment dog'') \citep{Murphy1988,Murphy2002}, unlike standard machine classifiers which are limited to a fixed set of classes
(``dog'', ``cat'', etc.).  Further, humans can induce ``ad hoc'' categories based on goals such as
``things to take from one's apartment in a fire'' (children, dogs, keepsakes, etc.)~\citep{Barsalou1983-ud}. Thus, unlike AI systems, humans reason seamlessly in large, essentially ``unbounded'' concept
spaces.

Beyond unboundedness, a natural challenge in such concept spaces
is \emph{uncertainty} -- the right concept to be
inferred is uncertain, as a plethora of candidate concepts could
explain observations. For \eg in ~\cref{fig:teaser} (top, image panel)
the ``right'' concept could be that ``All objects are blue and have
the same size'', but could also be ``There are less than four
objects in the scene'', or ``All objects have the same color''.
Humans gracefully handle such uncertainty and underdetermination \cite{Tenenbaum2001,Xu2007,Goodman2008a,Piantadosi2016-bx}.
%Building machines with productive concept learning would represent a major step forward.

This paper examines how modern machine learning systems can perform
more human like reasoning, leveraging compositionality to instantiate an
unbounded, productive concept space. Unlike previous related works in compositionality
~\citep{santoro_neurips2017,Johnson2016} our key focus is on
concept learning -- where a machine must acquire a concept
from finite samples, reason under uncertainty and induce abstract internal
representations.
We contribute the Productive Concept Learning (\pcl) benchmark for few-shot learning of relational concepts in a large compositional conceptual
space. \pcl includes scene-based concepts such as ``All objects have the same color'' and ``There exists a blue object while the rest are triangles'' (\cref{fig:teaser}), but unlike CLEVR \cite{Johnson2016_clevr} and related deductive reasoning tasks such as Ravens Progressive Matrices~\citep{santoro_neurips2017} there are too few examples to deduce answers with certainty -- meaning the ``concept'' or ``question'' to be answered is not given, but must
be inferred under uncertainty.

Our benchmark is defined through a series of meta-learning episodes (see example in \cref{fig:task}): given positive and negative examples of a new concept $D_{\text{supp}}$ (known as the ``support set''), the goal of an episode is to classify new examples $D_{\text{query}}$ (the ``query set''). As in few-shot classification \citep{FeiFeiFergus2006,LakeOmniglotProgress,Mordatch2018-gn}, meta-learning \citep{Vinyals2016-ri,Santoro2016-ug,Snell2017-rl,Grant2019a}, and other open-set tasks \citep{Scheirer2013-ho,Lampert2014-qo}, models are evaluated on novel classes outside the (meta-)training set. Unlike previous work~\citep{meta_dataset,LakeOmniglotProgress} that focuses on atomic concepts, our benchmarks concerns more structured, relational concepts built compositionally from a set of atomic concepts, and involves
reasoning under uncertainty -- an ideal learner must marginalize over many hypotheses when making predictions \citep{Gelman2004,Tenenbaum2001,Xu2007,Piantadosi2016-bx}. Finally, we also vary the modality in which scenes are presented---rendering them as images, symbolic schemas, and sounds--- further emphasizing abstract reasoning over the particulars of the input representation.

Our choice of compositional concepts was most closely inspired by \citep{Piantadosi2016-bx} along with other studies of human concept learning in the Language of Thought (LOT) framework~\citep{Fodor1975,Goodman2008a,Kemp2009-sn,Piantadosi2012,Goodman2014,Overlan2017,LakeFractals2019}. In typical LOT studies of human learning, the conceptual space $\calH$ is defined through a probabilistic context-free grammar $\calG$, which specifies a set of conceptual primitives and their rules of combination. 
%Not only does $\calG$ generate the stimuli, it is often used for cognitive modeling; learning is operationalized as a Bayesian search through the LOT for the best descriptions of the examples. Our goals differ here; 
Here, we use a LOT-inspired grammar $\calG$ to generate an unbounded set concepts $\calH$, while evaluating machine learning models trained without access to the underlying LOT.

A critical feature of our work is a set of train/validation/test splits which evaluate different notions of systematic generalization, an ability that has historically challenged neural networks \cite{Fodor1988,Marcus2003} and continues to challenge them in today's benchmarks~\citep{Barrett2018-qr,Hill2019-as,Agrawal2017-qw,Johnson2016_clevr,imagination,Higgins2017-wa,Bakhtin2019-sy,LakeBaroni2018,Ruis2020}. Concretely, our benchmark evaluates how models generalize to more complex or
productive concepts and novel combinations than seen during training, including novel combinations of intrinsic properties (\eg color shape) with boolean operators, counting, extrinsic object properties (\eg object location), and variable binding (binding a novel predicate ``blue'' with the abstract notion of color).

In addition to defining such splits we characterize the difficulty
of generalization entailed by each split by introducing the notion
of a model-independent ``compositionality gap''. Concretely, the compositionality gap is the difference in test performance between an ideal Bayesian learner with access to the full hypothesis space (e.g., the LOT), and a Bayesian learner with access to only a (potentially large) list of the hypotheses examined during meta-training. A large gap indicates that any learner must extrapolate compositionally from the training hypotheses to solve the task; additionally, models can be compared to ideal learners that either do or do not engage in such extrapolation. We anticipate that this tool will be more broadly useful for analyzing other benchmarks with compositional splits.

%We offer a `compositionality gap' metric for systematic generalization as another key contribution of our work (\cref{sec:metrics}). 
%Another contribution of this work is the introduction of a model-independent measure for evaluating the difficulty of generalizing to novel compositional concepts $\calH_{test}$ (during meta-test) based on prior experience with a different set of concepts $\calH_{train}$ (during meta-training). Concretely, the compositionality gap is the difference in test performance between an ideal Bayesian learner with access to the full hypothesis space (e.g., the LOT), and a Bayesian learner with access to only a (potentially large) list of the hypotheses examined during meta-training ($\calH_{train}$).  The combination of our systematic splits and associated compositionality gaps illuminate the successes and failures of current models. We anticipate that this tool will be more broadly useful for analyzing other benchmarks with compositional splits.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_v2.pdf}
    \caption{\noindent\textbf{Concept Space}. Three example concepts (rows)  along with schematic positive examples. Actual scenes are rendered  in multiple ways including the CLEVR renderer \citep{Johnson2016_clevr} (see \cref{fig:task}).
    \textbf{Right:} The grammar of variables, quantifiers, functions and operators to induce compositional concepts. }
    \label{fig:teaser}
\end{figure}
    % \ari{I'm worried readers are going to think that these 2D scenes are what the actual dataset looks like. Can we replace with real images? Perhaps we could merge this with \cref{fig:task} by showing 2 positive and 2 negative examples for each?}

We evaluate a broad range of baseline models on versions of \pcl rendered in different modalities. This includes meta-learning models \cite{Snell2017-rl} operating over different architectures for reasoning about objects in scenes. We also evaluate models trained to predict classification labels and symbolic (LOT) descriptions at training time, and those that are only trained to predict classification labels. Overall, our evaluations suggest that there is
substantial room for improvement in machine compositional
reasoning w.r.t the compositionality gap, and hope our benchmark
serves to help close that gap.

\noindent\textbf{Summary of contributions:}
1) We introduce the Productive Concept Learning (\pcl) benchmark for evaluating compositional, relational learning from observational data; 
2) We introduce a `compositionality gap' metric for measuring the difficulty of systematic generalization from train to test;
3) We provide baseline models to facilitate future work on our challenges.
